The Effect of Saturation on Belief Propagation Decoding of LDPC Codes

We consider the effect of LLR saturation on belief propagation decoding of low-density parity-check codes. Saturation occurs universally in practice and is known to have a significant effect on error floor performance. Our focus is on threshold analysis and stability of density evolution. We analyze the decoder for certain low-density parity-check code ensembles and show that belief propagation decoding generally degrades gracefully with saturation. Stability of density evolution is, on the other hand, rather strongly affected by saturation and the asymptotic qualitative effect of saturation is similar to reduction of variable node degree by one.

==> definitions.tex <==
% The following commands allow CVS to insert the
% current information regarding this file:
% ----------------------------------------------
% $RCSfile$
% $Date: 2009-12-14 15:21:24 +0100 (Mon, 14 Dec 2009) $
% $Author: ruediger $
% $Revision: 1552 $
% $Source$
% $State$
% -----------------------------------------------
% Commands for theorems and such
% ------------------------------
%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{example}{Example}[chapter]
%\newtheorem{proposition}{Proposition}[chapter]
%\newtheorem{conjecture}{Conjecture}[chapter]
%\newtheorem{fact}{Fact}[chapter]
%\theoremstyle{definition}
%\newtheorem{exercise}{}[chapter]
\newcommand{\Exercises}{\section*{\centering Exercises}\addcontentsline{toc}{section}{\numberline{}Exercises}\markright{\footnotesize EXERCISES}}
\newcommand{\History}{\section*{\centering Notes}\addcontentsline{toc}{section}{\numberline{}Notes}\markright{\footnotesize NOTES}}
\newcommand{\btheorem}{\begin{theorem}\rm}
\newcommand{\etheorem}{\end{theorem}}
\newcommand{\bcorollary}{\begin{corollary}\rm}
\newcommand{\ecorollary}{\end{corollary}}
\newcommand{\bconjecture}{\begin{conjecture}\rm}
\newcommand{\econjecture}{\end{conjecture}}
\newcommand{\blemma}{\begin{lemma}\rm}
\newcommand{\elemma}{\end{lemma}}
\newcommand{\bdefinition}{\begin{definition}\rm}
\newcommand{\edefinition}{\end{definition}}
\newcommand{\bexample}{\begin{example}\rm}
\newcommand{\eexample}{\end{example}}
\newcommand{\bproposition}{\begin{proposition}\rm}
\newcommand{\eproposition}{\end{proposition}}
\newcommand{\bfact}{\begin{fact}\rm}
\newcommand{\efact}{\end{fact}}
\newcommand{\bexercise}{\begin{exercise}\rm}
\newcommand{\eexercise}{\end{exercise}}
\newcommand{\EEx}{\hfill $\Box$}
\newcommand{\EDe}{\hfill $\clubsuit$}

% algebraic objects
%------------------
\DeclareMathOperator{\reals}{\ensuremath{\mathbb{R}}}
\DeclareMathOperator{\realsplus}{\ensuremath{\mathbb{R}^+}}
\DeclareMathOperator{\creals}{\ensuremath{\bar{\mathbb{R}}}}
\DeclareMathOperator{\cR}{\creals}
\DeclareMathOperator{\crealsplus}{\ensuremath{\bar{\mathbb{R}}^+}}
\DeclareMathOperator{\cRp}{\crealsplus}
\DeclareMathOperator{\GF}{GF}
\DeclareMathOperator{\field}{\ensuremath{\mathbb{F}}}
\DeclareMathOperator{\F}{\field}
\DeclareMathOperator{\extensionfield}{\ensuremath{\mathbb{E}}}
\DeclareMathOperator{\semiring}{\ensuremath{\mathbb{K}}}
\DeclareMathOperator{\complex}{\ensuremath{\mathbb{C}}}
\DeclareMathOperator{\integers}{\ensuremath{\mathbb{Z}}}
\DeclareMathOperator{\naturals}{\ensuremath{\mathbb{N}}}
\DeclareMathOperator{\rationals}{\ensuremath{\mathbb{Q}}}

% operators 
% ---------
\DeclareMathOperator{\expectation}{\ensuremath{\mathbb{E}}} % expectation operator
%\DeclareMathOperator{\probability}{{\text{\rm P}}}    % alias
\DeclareMathOperator{\prob}{{\text{\rm P}}}    % generic probability
\DeclareMathOperator{\perr}{\mathfrak{E}}       % probability of error operator
\DeclareMathOperator{\batta}{\mathfrak{B}}      % Battacharya operator
\DeclareMathOperator{\fourier}{\mathfrak{F}}    % Fourier transform operator
\DeclareMathOperator{\harddec}{\mathfrak{H}}    % hard decision operation
\DeclareMathOperator{\w}{w}    % weight 


% generic code 
% ------------
\newcommand{\codeword}{{codeword}}
\newcommand{\dd}{dd} % degree distribution
\newcommand{\code}{C}
\newcommand{\dualcode}{C^{\perp}}
\newcommand{\generator}{G}
\newcommand{\parity}{H}
\newcommand{\gshannon}{{\cal G}}
\newcommand{\hshannon}{{\cal H}}
\newcommand{\capacity}{\text{C}}
\newcommand{\entropy}{\text{H}}

% Tanner graph 
% ------------
\newcommand{\graph}{{{\tt G}}}
\newcommand{\standardgraph}{\Gamma}
\newcommand{\standardgraphensemble}{{G}}
\newcommand{\complexgraph}[3]{{\cal G}_{#1}(#2, #3)}
\newcommand{\cnode}{{\tt c}}
\newcommand{\vnode}{{\tt v}}
\newcommand{\dr}{{\tt r}}
\newcommand{\dravg}{{\tt r}_{\text{avg}}}
\newcommand{\drmin}{{\tt r}_{\text{min}}}
\newcommand{\drmax}{{\tt r}_{\text{max}}}
\newcommand{\dl}{{\tt l}}
\newcommand{\dlavg}{{\tt l}_{\text{avg}}}
\newcommand{\dlmin}{{\tt l}_{\text{min}}}
\newcommand{\dlmax}{{\tt l}_{\text{max}}}
\newcommand{\Edges}{E}
\newcommand{\edge}{{{\tt e}}}
\newcommand{\codetensor}{f}
\newcommand{\hamiltonian}{E}

% algebraic notions
% -----------------
\newcommand{\group}{G}
\newcommand{\groupelement}{g}
\newcommand{\dualgroup}{\Gamma}
\newcommand{\character}{\gamma}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indicator}[1]{\ind_{\{ #1 \}}}
%\newcommand{\defeq}{\stackrel{\vartriangle}{=}}
\newcommand{\defeq}{\triangleq}
\newcommand{\myscriptsize}{\tiny}

% Tree codes 
% ----------
\newcommand{\treeensemble}{{\cal T}}
\newcommand{\ctreeensemble}{{\cal C}}
\newcommand{\nodetreeensemble}{\dot{\cal T}}
\newcommand{\edgetreeensemble}{\vec{\cal T}}
\newcommand{\nodectreeensemble}{\dot{\cal C}}
\newcommand{\edgectreeensemble}{\vec{\cal C}}
\newcommand{\tree}{{{\tt T}}}
\newcommand{\ltree}{{{\tt L}}}
\newcommand{\rtree}{{{\tt R}}}
\newcommand{\minimal}{{{\cal P}}}

% LDPC ensembles 
% --------------
\newcommand{\ensemble}[3]{{\cal C}\left(#1, #2, #3 \right)}
\newcommand{\nldpc}[2]{\text{LDPC}\left(#1, #2 \right)}
\newcommand{\eldpc}[3]{\text{LDPC}\left(#1, #2, #3 \right)}
\newcommand{\peldpc}[4]{\text{LDPC}\left(#1, #2, #3, #4 \right)}
\newcommand{\nsldpc}[2]{\text{LDPC}_{<}\left(#1, #2 \right)}
\newcommand{\esldpc}[3]{\text{LDPC}_{<}\left(#1, #2, #3 \right)}
\newcommand{\nrldpc}[2]{\text{LDPC}_{\circ}\left(#1, #2 \right)}
\newcommand{\erldpc}[3]{\text{LDPC}_{\circ}\left(#1, #2, #3 \right)}
\newcommand{\ldpcp}[2]{\text{LDPC}_{P}\left(#1, #2 \right)}
\newcommand{\ldpc}[3]{\text{LDPC}\left(#1, #2, #3 \right)}
\newcommand{\epldpc}[3]{\text{LDPC}_{P}\left(#1, #2, #3\right)}
\newcommand{\npldpc}[2]{\text{LDPC}\left(#1, #2 \right)}
\newcommand{\ledge}{\lambda}           % left degree distribution-edge perspective
\newcommand{\redge}{\rho}              % right degree distribution-edge perspective
%\newcommand{\densredge}[1]{\Gamma^{-1}(\redge(\Gamma(#1)))}
\newcommand{\densredge}[1]{\redge(#1)} % density form with Gamma dropped
\newcommand{\lnode}{\Lambda}           % left degree distribution-node perspective
\newcommand{\lnodenormalized}{L}           % left degree distribution-node perspective and normalized
\newcommand{\lnoden}{\lnodenormalized}     % left degree distribution-node perspective and normalized
\newcommand{\rnode}{P}                 % right degree distribution-node perspective
\newcommand{\rnodenormalized}{R}                 % right degree distribution-node perspective normalized
\newcommand{\rnoden}{\rnodenormalized}                 % right degree distribution-node perspective normalized
%\newcommand{\ledger}{\underline{\lambda}}           % left degree distribution-edge perspective
%\newcommand{\redger}{\underline{\rho}}              % right degree distribution-edge perspective
%\newcommand{\lnoder}{\underline{\Lambda}}           % left degree distribution-node perspective
%\newcommand{\rnoder}{\underline{P}}                 % right degree distribution-node perspective
\newcommand{\ddeq}{\circeq}                % equalilty of degree distributions in different representations

\newcommand{\ledger}{\lambda}           % left degree distribution-edge perspective
\newcommand{\redger}{\rho}              % right degree distribution-edge perspective
\newcommand{\lnoder}{\Lambda}           % left degree distribution-node perspective
\newcommand{\rnoder}{P}                 % right degree distribution-node perspective
\newcommand{\redgedev}{\delta}              % right degree distribution-edge perspective
\newcommand{\rnodedev}{\Delta}                 % right degree distribution-node perspective
\newcommand{\redgedom}{\gamma}              % right degree distribution-edge perspective
\newcommand{\rnodedom}{\Gamma}                 % right degree distribution-node perspective

\newcommand{\CtoV}{{\tt left-to-right }}
\newcommand{\VtoC}{{\tt right-to-left }}

% iterative decoder 
% -----------------
\newcommand{\iterations}{\ell}
\newcommand{\iteration}{\ell}
\newcommand{\erasureset}{{\cal E}}
\newcommand{\eset}{{\cal E}}
\newcommand{\kset}{{\cal K}}

% EXIT Charts
% -----------
\newcommand{\exitf}{h}
\newcommand{\exitF}{H}

% stopping sets etc. 
% ------------------
\newcommand{\total}{T}
\newcommand{\Total}{{\cal T}}
\newcommand{\stopping}{S}
\newcommand{\none}{N}
\newcommand{\None}{{\cal N}}
\newcommand{\bad}{B}
\newcommand{\Bad}{{\cal B}}
\newcommand{\ssmin}{s_{\text{min}}}
\newcommand{\ssmax}{s_{\text{max}}}
\newcommand{\ssmaximal}{s}

% mbs channels 
% ------------
\newcommand{\channelto}[1]{\xrightarrow{\quad #1 \quad}}
\newcommand{\smallchannelto}[1]{\xrightarrow{\; #1 \;}}
\newcommand{\channelfrom}[1]{\xleftarrow{\quad #1 \quad}}
\newcommand{\inalphabet}{{\cal X}} % channel input alphabet 
\newcommand{\out}{{\cal Y}}        % chanel output alphabet
\newcommand{\llr}{l}   % log-likelihood ratio
\newcommand{\Llr}{L}   % log-likelihood ratios as a rv
\newcommand{\diffp}{D}   % log-likelihood ratios as a rv
\newcommand{\delinf}{\Delta_{\infty}}  % delta function at infinity
\newcommand{\delzero}{\Delta_{0}}      % delta function at zero
%\newcommand{\conv}{\otimes}
\newcommand{\conv}{\star}
\newcommand{\physicallypreceeds}{\prec}
\newcommand{\physicallysucceeds}{\succ}

% density and distribution macros
%------------------
%\newcommand{\channel}[1]{\mathit{\MakeLowercase{#1}}}
\newcommand{\channel}[1]{\MakeLowercase{#1}}
\newcommand{\abs}[1]{{\lvert #1 \rvert}}
\newcommand{\absd}[1]{|#1|}
\newcommand{\spaceofLdistributions}{{\cal A}_{L}}
\newcommand{\spaceofabsLdistributions}{{\cal A}_{\absd{L}}}
\newcommand{\spaceofDdistributions}{{\cal A}_{D}}
\newcommand{\spaceofabsDdistributions}{{\cal A}_{\absd{D}}}
\newcommand{\spaceofGdistributions}{{\cal A}_{G}}
\newcommand{\Ddistribution}{$D$-distribution}
\newcommand{\absDdistribution}{$\absd{D}$-distribution}
\newcommand{\Ldistribution}{$L$-distribution}
\newcommand{\absLdistribution}{$\absd{L}$-distribution}
\newcommand{\Gdistribution}{$G$-distribution}
\newcommand{\Ddistributions}{$D$-distributions}
\newcommand{\absDdistributions}{$\absd{D}$-distributions}
\newcommand{\Ldistributions}{$L$-distributions}
\newcommand{\Gdistributions}{$G$-distributions}
\newcommand{\absGdistribution}{$\absd{G}$-distribution}
\newcommand{\absLdistributions}{$\absd{L}$-distributions}
\newcommand{\Ldensity}{$L$-density}
\newcommand{\absLdensity}{$\absd{L}$-density}
\newcommand{\Ddensity}{$D$-density}
\newcommand{\Gdensity}{$G$-density}
\newcommand{\absDdensity}{$\absd{D}$-density}
\newcommand{\absDdensities}{$\absd{D}$-densities}
\newcommand{\Ldensities}{$L$-densities}
\newcommand{\Ddensities}{$D$-densities}
\newcommand{\Gdensities}{$G$-densities}
\newcommand{\absLdensities}{$\absd{L}$-densities}
\newcommand{\vect}[1]{{\underline{#1}}}
\newcommand{\vectbs}[1]{{\underline{#1}}}

% generic distributions and densities
\newcommand{\dist}[1]{\mathsf{\MakeUppercase{#1}}}
\newcommand{\absdist}[1]{\absd{\dist{#1}}}
\newcommand{\dens}[1]{\mathsf{\MakeLowercase{#1}}}
\newcommand{\absdens}[1]{\absd{\dens{#1}}}
\newcommand{\heaviside}{\dist{H}}             % heaviside function
\newcommand{\ddist}[1]{\,d \dist{#1}}  % distribution
\newcommand{\vLdens}[1]{\underline{\dens{#1}}} % vector of densities
% L distributions and densities
\newcommand{\Ldist}[1]{\dist{#1}}
\newcommand{\absLdist}[1]{\absdist{#1}}
\newcommand{\Ldens}[1]{\dens{#1}}
\newcommand{\absLdens}[1]{\absdens{#1}}
% D distributions and densities
\newcommand{\Ddist}[1]{\mathfrak{\MakeUppercase{#1}}}
\newcommand{\absDdist}[1]{\absd{\mathfrak{\MakeUppercase{#1}}}}
\newcommand{\Ddens}[1]{\mathfrak{\MakeLowercase{#1}}}
\newcommand{\absDdens}[1]{\absd{\Ddens{#1}}}
% G distributions and densities
\newcommand{\Gdist}[1]{\mathit{\MakeUppercase{#1}}}
\newcommand{\absGdist}[1]{\absd{\mathit{\MakeUppercase{#1}}}}
\newcommand{\Gdens}[1]{\mathit{\MakeLowercase{#1}}}
\newcommand{\absGdens}[1]{\absd{\Ddens{#1}}}

% other stuff
\newcommand{\pdiff}{d}
\newcommand{\lgpdiff}{g}
\newcommand{\gmap}{\Gamma}
\newcommand{\Pdiff}{D}

% for proof of physical degradation theorem
\newcommand{\ugf}{u_{\text{\myscriptsize GF}}}
\newcommand{\ufg}{u_{\text{\myscriptsize FG}}}
\newcommand{\Afg}{A_{\text{\myscriptsize FG}}}
\newcommand{\Agf}{A_{\text{\myscriptsize GF}}}
\newcommand{\zAgf}{\hat{A}_{\text{\myscriptsize GF}}}
\newcommand{\zpm}{z_{\uparrow}}
\newcommand{\invzpm}{z^{-1}_{\uparrow}}
\newcommand{\invF}{{\absDdist{F}}^{-1}}
\newcommand{\invG}{{\absDdist{G}}^{-1}}

% picture macros
%
\newcommand{\nudge}[3]{\hspace{#1 pt}\raisebox{#2 pt}{#3}}
% junk macros 
% -----------
\newcommand{\sfield}{{\cal F}}
\newcommand{\dneigh}[2]{{\cal N}_{#1}^{#2}}
\newcommand{\rec}{{\tt r}}
\newcommand{\neigh}[2]{{\cal N}_{#1}^{#2}}
\newcommand{\gf}{\hat{\gamma}}
\newcommand{\sset}{{\cal S}}
\newcommand{\lset}{{\cal V}}
\newcommand{\rset}{{\cal C}}
\newcommand{\vset}{{\cal V}}
\newcommand{\e}{e}
\newcommand{\mue}{\mu}
\newcommand{\nue}{\nu}
\DeclareMathOperator{\degreefunction}{{\cal D}}
\DeclareMathOperator{\normalizeddegreefunction}{{\cal N}}
\newcommand{\tindex}{t}
\newcommand{\outp}{y}
\newcommand{\inp}{{\tt x}}
\newcommand{\cnd}{{\tt c}}
\newcommand{\mesg}{\mu}
\newcommand{\vnd}{{\tt v}}
%\newcommand{\vnd}[1]{\vnode_{#1}}
\def\Plo{\vnd_{\ell-1}}
\def\Rlo{\cnd_{\ell-1}}
\newcommand{\vnodes}{{{\cal V}}}
\newcommand{\cnodes}{{{\cal C}}}
\newcommand{\allone}{\vect{1}}
\newcommand{\oa}{{\cal O}}
\newcommand{\ma}{{\cal M}}
\newcommand{\node}{{\tt u}}
%\newcommand{\vmessagemap}[1]{\Psi_{\tt v}^{(#1)}}
%\newcommand{\cmessagemap}[1]{\Psi_{\tt c}^{(#1)}}
\newcommand{\vmessagemap}[1]{\Psi^{(#1)}}
\newcommand{\cmessagemap}[1]{\Phi^{(#1)}}
\newcommand{\prvmessagemap}[1]{{{}^\star\Psi}_{\tt v}^{(#1)}}
\newcommand{\prcmessagemap}[1]{{{}^\star\Psi}_{\tt c}^{(#1)}}
\newcommand{\oquan}{{q_o}}
\newcommand{\quan}{q}
\newcommand{\x}{{\tt x}}
\newcommand{\p}[2]{p_{#1}^{(#2)}}
\newcommand{\dedge}{\vec{\tt e}}
\newcommand{\q}[2]{q_{#1}^{(#2)}}
\newcommand{\vmsgmap}{\Psi_{\tt v}}
\newcommand{\cmsgmap}{\Psi_{\tt c}}
\newcommand{\mesn}[1]{\vnode_{#1}}
\newcommand{\chen}[1]{\cnode_{#1}}
\newcommand{\sign}{\ensuremath{\mathsf{sgn}\,}}
\newcommand{\simplegraph}{{\cal G}}
\newcommand{\prcmsgmap}{{{}^\star\Psi}_{\tt c} }
\newcommand{\prvmsgmap}{{{}^\star\Psi}_{\tt v} }
\DeclareMathOperator{\fnode}{{\tt f}}
\DeclareMathOperator{\unode}{{\tt u}}
\DeclareMathOperator{\gnode}{{\tt g}}
\DeclareMathOperator{\edges}{E}
\DeclareMathOperator{\neighbors}{N}
\newcommand{\correct}{{\cal G}}
\newcommand{\erroneous}{{\cal B}}
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\iterlim}{{\stackrel{\iteration \rightarrow \infty}{\longrightarrow}}}

% reed solomon codes
\newcommand{\spa}{A}
\newcommand{\spb}{B}
\newcommand{\spc}{C}
\newcommand{\chord}{S}

% stability paper
\newcommand{\ptree}{t}
\newcommand{\primsubtrees}{\Psi (T)}
\newcommand{\vnoderoot}{{\tt v}_{\text{\small root}}}
\newcommand{\droot}{d_{\text{\small root}}}
\newcommand{\smvnoderoot}{{\tt v}_{\text{\tiny root}}}
%\newcommand{\smprec}{P_{\text{\small rec}}}
%\newcommand{\perr}{\prob_{\text{\small err}}}
\newcommand{\tg}{\tilde{g}}
\renewcommand{\th}{\beta}
%\newcommand{\qleaf}{q_{\cal Q}}

\newcommand{\alphabet}{{\cal A}}
\newcommand{\alphabetsize}{A}
\def\llim{\lim_{x \rightarrow -\infty}}
\def\rlim{\lim_{x \rightarrow +\infty}}
\def\infpm{(-\infty,+\infty]}
\newcommand{\dominant}{{\cal D}}
\newcommand{\intlambda}{\text{$\int \!\! \lambda$}\;}
\newcommand{\intrho}{\text{$\int \!\! \rho$}\;}
\newcommand{\xzs}{\underline{x_0^{*}}}
\newcommand{\intrhomin}{\underline{\text{$\int \!\! \rho$}}\;}
\newcommand{\lambdatwomax}{\overline{\lambda_2}}
\newcommand{\intrhomax}{\overline{\text{$\int \!\! \rho$}}\;}
\newcommand{\ovi}{{\textstyle \frac{1}{i}}}
\newcommand{\ovip}{{\textstyle \frac{1}{i+1}}}
\newcommand{\ccns}{\text{$\int \!\! \lambda$}\;}
\newcommand{\ovj}{{\textstyle \frac{1}{j}}}
\newcommand{\ic}{\left(\ovi-\ccns\right)}
\newcommand{\omrji}{(1-r)^{j-i}}
\newcommand{\omr}{(1-r)}
\newcommand{\rji}{r^{j-i}}
\newcommand{\cip}{\left(\ccns-\ovip\right)}
\newcommand{\cj}{\left(\ccns-\ovj\right)}
\newcommand{\omrjip}{(1-r)^{j-i+1}}
\newcommand{\rjip}{r^{j-i+1}}
\def\Q{\text{$\cal Q$}}
\newcommand{\intrhomint}{\underline{\text{$\int \!\! \tilde{\rho}$}}\;}
\newcommand{\wst}{{\tt t}}
\newcommand{\wsv}{{\tt v}}
\newcommand{\centert}{{\tt T}}
\newcommand{\centerv}{{\tt V}}

\def\pl{x_\ell} % erasure probability at l-th round of BP on Erasure
                % Channel
\def\plo{x_{\ell-1}}
\def\Pl{\vnd_\ell} % Density of the messages sent from variable nodes to
                % check nodes at l-th round of the BP
\newcommand{\Rl}{a} % Density of messages sent from check nodes to
\newcommand{\distPl}{\int\!\vnd_{\ell}} % Density of the messages sent from variable nodes to
\newcommand{\distRl}{\int\! \cnd_{\ell}} % Density of messages sent from check nodes to
\newcommand{\distRlo}{\int\! \cnd_{\ell-1}}
\def\atanh{\mathrm{atanh}}
\def\vn{variable node}
\def\cn{check node}
\def\sgn{\mathrm{sgn}}

\def\L{\mathrm{L}} % \L(y) is the likelihood ratio of y

\def\indass{{\em independence assumption}}
%\def\BP{{\em belief-propagation}}

\newcommand{\mydeltat}{e}
\newcommand{\mydeltas}{c}
\newcommand{\mysigma}{d}
\newcommand{\mytau}{f}
\newcommand{\deltat}{\Delta t}
\newcommand{\deltas}{\Delta s}
\newcommand{\tdrift}{\text{f}_{t}}
\newcommand{\sdrift}{\text{f}_{s}}
\newcommand{\tvariance}{\text{f}_{t,t}}
\newcommand{\svariance}{\text{f}_{s,s}}
\newcommand{\tsvariance}{\text{f}_{t,s}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\infpm{(-\infty,+\infty]}
\def\llim{\lim_{x \rightarrow -\infty}}
\def\rlim{\lim_{x \rightarrow +\infty}}
\def\lgsgn{\sgn}
\def\mvc{{\tt m}_{\tt vc}} % Message sent from variable node v to check node c
\def\mvcl{\mvc^{(\ell)}}
\def\mvcl{\mvc^{(\ell)}}
\def\mcv{{\tt m}_{\tt cv}} % Message sent from check node c to variable node v
\def\mcvl{\mcv^{(\ell)}}
\def\scv{s_{cv}} % Sign
%\def\dx{\,\d x}
%\def\dy{\,\d y}
%\def\dz{\,\d z}
\def\dx{{\, d \! x}}
\def\dy{{\, d \! y}}
\def\dz{{\, d \! z}}
\def\dpp{{\, d \! p}}
\def\deps{{\, d \! \epsilon}}
\def\tensor{\star}
%\newcommand{\delinf}{\Delta_{\infty}}
\def\distRl{\int\! \cnd_{\ell}} % Density of messages sent from check nodes to
\def\distRlo{\int\! \cnd_{\ell-1}}
\def\distPl{\int\!\vnd _\ell} % Density of the messages sent from variable nodes to
                % check nodes at l-th round of the BP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% turbo code section
\newcommand{\demaps}[3]{\Gamma_{#3}^s(#1, #2)}  % map between densities for trellis: sytematic bits
\newcommand{\demapp}[3]{\Gamma_{#3}^p(#1, #2)}  % map between densities for trellis: parity bits
\newcommand{\demap}[3]{\Gamma_{#3}(#1, #2)}  % map between densities for trellis: either
\newcommand{\demapsshort}[2]{\Gamma^s(#1, #2)}  % map between densities for trellis: sytematic bits
\newcommand{\demappshort}[2]{\Gamma^p(#1, #2)}  % map between densities for trellis: parity bits
\newcommand{\demapshort}[2]{\Gamma(#1, #2)}  % map between densities for trellis: either
\newcommand{\iw}{i}   % input weight; weight of systematic bits
\newcommand{\ow}{o}   % output weight; weight of parity bits
\newcommand{\tw}{w}   % weight of all bits; total weight
\newcommand{\state}{\sigma}   % state of a trellis, i.e., content of shift register 
\newcommand{\State}{\Sigma}   % same as state but if considered as random variable 
\newcommand{\gfc}{C}   % generating function for weight distribution: convolutional code 
\newcommand{\gfp}{P}   % generating function for weight distribution: parallel concatenated code 
\newcommand{\gfs}{S}   % generating function for weight distribution: serially concatenated code
\newcommand{\gfpasym}{\bar{P}}   % generating function for weight distribution: parallel concatenated code
\newcommand{\gfsasym}{\bar{S}}   % generating function for weight distribution: serially concatenated code
\newcommand{\gfpasymp}{\tilde{P}}   % generating function for weight distribution: parallel concatenated code
\newcommand{\gfsasymp}{\tilde{S}}   % generating function for weight distribution: serially concatenated code
\newcommand{\cgfc}{c}   % coefficient of generating function for weight distribution: convolutional code
\newcommand{\cgfp}{p}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfs}{s}   % coefficient of generating function for weight distribution: serially concatenated code
\newcommand{\gfdet}{D}   % generating function of detours
\newcommand{\cgfpasym}{\bar{p}}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfsasym}{\bar{s}}   % coefficient of generating function for weight distribution: serially concatenated code
\newcommand{\cgfpasymp}{\tilde{p}}   % coefficient of generating function for weight distribution: parallel concatenated code
\newcommand{\cgfsasymp}{\tilde{s}}   % coefficient of generating function for weight distribution: serially concatenated cod
\newcommand{\mat}{M}   % matrix for transfer matrix method 
\newcommand{\matfinal}{\bar{M}}   % matrix for transfer matrix method for the last m steps
\newcommand{\matdet}{M^{\bullet}}   % matrix for transfer matrix method to compute detours 


\newcommand {\barr}{\begin{array}}
\newcommand {\earr}{\end{array}}

% covariance evolution
\newcommand{\ebar}{\overline{\epsilon}}
\newcommand{\Sur}{P_{\rm S}}
\newcommand{\Wh}{\widehat{W}}
\newcommand{\Xh}{\widehat{X}}
\newcommand{\Ph}{\widehat{P}}
\newcommand{\oX}{\overline{X}}
\newcommand{\oz}{\overline{z}}
\newcommand{\oth}{\overline{\theta}}
\newcommand{\fh}{\hat{f}}
\newcommand{\Dh}{\widehat{D}}
\newcommand{\Wt}{\widetilde{W}}
\newcommand{\Hp}{{\mathbb H}_+}
\newcommand{\R}{{\mathbb R}}
\newcommand{\vD}{\vec{\Delta}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vX}{\vec{X}}
\newcommand{\vz}{\vec{z}}
\newcommand{\Ai}{{\rm Ai}}
\newcommand{\Bi}{{\rm Bi}}
\newcommand{\ve}{\varepsilon}
%\newcommand{\ledger}{\lambda}           % left degree distribution-edge perspective
%\newcommand{\redger}{\rho}              % right degree distribution-edge perspective
%\newcommand{\lnoder}{\Lambda}           % left degree distribution-node perspective
%\newcommand{\rnoder}{P}                 % right degree distribution-node perspective
%\newcommand{\redgedev}{\delta}              % right degree distribution-edge perspective
%\newcommand{\rnodedev}{\Delta}                 % right degree distribution-node perspective
%\newcommand{\redgedom}{\gamma}              % right degree distribution-edge perspective
%\newcommand{\rnodedom}{\Gamma}                 % right degree distribution-node perspective
\newcommand{\xl}{x_{l}}
\newcommand{\xr}{x_{r}}
\newcommand{\xleft}{x_{l}}
\newcommand{\xright}{x_{r}}

% Macros from Changyan
\newcommand{\ensembleldpc}[3]{{\cal C}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\expurgatedensembleldpc}[4]{{\cal C}^{ex}_{\text{LDPC}}(#1,#2, #3,#4)}
\newcommand{\separateensembleldpc}[4]{{\cal C}^{#4<}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\ensembleldpcstatphys}[3]{{\cal C}^{\text{sp}}_{\text{LDPC}}(#1,#2, #3)}
\newcommand{\ensembleira}[3]{{\cal C}_{\text{IRA}} (#1,#2, #3)}
\newcommand{\ensemblesira}[3]{{\cal C}_{\text{SIRA}} (#1,#2, #3)}
\newcommand{\ensemblensira}[3]{{\cal C}_{\text{NSIRA}} (#1,#2, #3)}

% macros for graphs
\newcommand{\graphtextsizelarge}{\normal}
\newcommand{\graphtextsize}{\small}
\newcommand{\graphtextsizesmall}{\footnotesize}
\newcommand{\degd}{dd}
\newcommand{\azumaalpha}{\gamma}
\renewcommand{\mid}{\,|\,}

% formal power sums
% -----------------
\newcommand{\indet}{D}    % indeterminated of a formal power sum
\newcommand{\fps}{F}      % standard formal power sum
\newcommand{\fpstwo}{G}   % standard formal power sum
\newcommand{\fpsthree}{H} % standard formal power sum

% abbreviations for sub and superscripts
% --------------------------------------
\newcommand{\cw}{{\text{\myscriptsize cw}}}
\newcommand{\sss}{{\text{\myscriptsize ss}}}
\newcommand{\MAP}{{\text{\myscriptsize MAP}}}
\newcommand{\ML}{{\text{\myscriptsize ML}}}
\newcommand{\IT}{{\text{\myscriptsize IT}}}
\newcommand{\BP}{{\text{\myscriptsize BP}}}
\newcommand{\EXIT}{EXIT}
\newcommand{\GEXIT}{GEXIT}

